Method for real-time monitoring of paramagnetic reactions using spin relaxometry with fluorescent nanodiamonds

Spin relaxometry using fluorescent nanodiamonds (FNDs) has been applied successfully to sense numerous paramagnetic target molecules such as free radicals and metalloproteins. However, despite their high sensitivity, T1 spin relaxation measurements are often hampered by their slow acquisition speed. Here, we demonstrate a method that allows for real-time monitoring of paramagnetic chemical reactions. We demonstrate T1 spin relaxometry from thousands of FNDs using an optimised cuvette-based system integrating an avalanche photodiode operated in linear mode, and a fast, fieldprogrammable gate array (FPGA) for data collation. We demonstrate chemical monitoring of the reduction of Cu(II) to Cu(I) ions in-solution with a 15 second integration using an optimised T1 sensing protocol. Our method achieves more than two orders of magnitude speed up with an order of magnitude reduction in cost when compared with traditional techniques. With further technical improvements, we believe this in-solution method could be extended to sense the sub-second chemical kinetics of paramagnetic molecules in solution.

==> latexmkrc <==
## this document is for referenceing sup info tables and figures
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
